Trimming Mobile Applications for Bandwidth-Challenged Networks in Developing Regions

Despite continuous efforts to build and update network infrastructure, mobile devices in developing regions continue to be constrained by limited bandwidth. Unfortunately, this coincides with a period of unprecedented growth in the size of mobile applications. Thus it is becoming prohibitively expensive for users in developing regions to download and update mobile apps critical to their economic and educational development. Unchecked, these trends can further contribute to a large and growing global digital divide. Our goal is to better understand the source of this rapid growth in mobile app code size, whether it is reflective of new functionality, and identify steps that can be taken to make existing mobile apps more friendly bandwidth constrained mobile networks. We hypothesize that much of this growth in mobile apps is due to poor resource/code management, and do not reflect proportional increases in functionality. Our hypothesis is partially validated by mini-programs, apps with extremely small footprints gaining popularity in Chinese mobile networks. Here, we use functionally equivalent pairs of mini-programs and Android apps to identify potential sources of "bloat," inefficient uses of code or resources that contribute to large package sizes. We analyze a large sample of popular Android apps and quantify instances of code and resource bloat. We develop techniques for automated code and resource trimming, and successfully validate them on a large set of Android apps. We hope our results will lead to continued efforts to streamline mobile apps, making them easier to access and maintain for users in developing regions.

==> related-work.tex <==
\section{Related Work}
\subsection{Necessity of light weight Android apps}

Resources of communication devices are always limited and precious, such as power to sensory infrastructure and memory or battery to smartphones. 
In many developing countries, there exist more severe limitations and shortages for communication infrastructures including the cloud{\color{red}~\cite{Helmer_DEV16}}. In the meanwhile, the mobile Internet users is growing rapidly, with the annual growth rate reaching 20.8\% in Egypt{\color{red}~\cite{Lazem_DEV16}}. 

%Storage is of vital importance to smartphones. [[ needs a ref to signify the degradation of performance with the increase of memory usage. ]] 
%Measurement results show that the average size of the apps are around **** MB [[Maybe could refer to the paper presented by Xiaolong.]] 
%Based on the studies by XXX, there are *** apps needed generally in one smartphone for one person [need ref from mobile CHI]. 
%In special, the storage space of popular smartphones are usually limited. The user experiences of uses in these countries are
%discounted heavily. 

%To deal with this problem, there have been a few efforts. There are designs aiming to realize 

